Cloud Cosmology : Building the Web Interface for iCosmo

Astronomy and cosmology have embraced the internet. We routinely and successfully use the internet as a repository for sharing code, publications and information, and as a computational resource. However the interactive nature of the web, for use as an alternative to downloading code has been largely overlooked. In this article we will outline a simple framework in which a cosmological code can be turned into an interactive web interface. This is presented as a result of creating http://www.icosmo.org which is a front-end for the open-source software iCosmo. We explain how an HTML page can be created and how a cosmological code can be incorporated into a web environment using CGI scripts. We outline how plots and downloadable text can be made, and describe how help and documentation can be created. By using simple HTML and CGI scripts a basic web interface for any cosmological code can be created easily. We provide a worked example of the methods outlined, which can be used as a simple template by any researcher who wants to share their work online.

==> listings/Makefile <==
# This file generates files required to use the listings package.
#
# (c) 2007 Brooks Moses
#
# This file is distributed under the terms of the LaTeX Project Public
# License from CTAN archives in directory  macros/latex/base/lppl.txt.
# Either version 1.3 or, at your option, any later version.

.PHONY: listings pdf pdf-devel all

listings: listings.sty

pdf: listings.pdf

pdf-devel: listings-devel.pdf

all: listings pdf pdf-devel


listings.sty: listings.dtx listings.ins lstdrvrs.dtx
	tex listings.ins

listings.pdf: listings.sty
	rm -f ltxdoc.cfg
	pdflatex listings.dtx
	makeindex -s gind.ist listings
	pdflatex listings.dtx
	pdflatex listings.dtx

listings-devel.pdf: listings.sty
	rm -rf ltxdoc.cfg
	echo "\AtBeginDocument{\AlsoImplementation}" > ltxdoc.cfg
	pdflatex -jobname=listings-devel listings.dtx
	makeindex -s gind.ist listings-devel
	pdflatex -jobname=listings-devel listings.dtx
	pdflatex -jobname=listings-devel listings.dtx
	rm -rf ltxdoc.cfg


==> listings/README <==
Listings package
Copyright 1996--2004 Carsten Heinz (the package)
Copyright 1996--2007 individual authors (language drivers)
Copyright 2006--2007 Brooks Moses (continued maintenance)
Released under the LaTeX Project Public License 1.3 or later

The `listings' package is a source code printer for LaTeX.
You can typeset stand alone files as well as listings with
an environment similar to `verbatim' as well as you can
print code snippets using a command similar to \verb'.
Many parameters control the output and if your preferred
programming language isn't already supported, you can make
your own definition.


==> listings/listings/Makefile <==
# This file generates files required to use the listings package.
#
# (c) 2007 Brooks Moses
#
# This file is distributed under the terms of the LaTeX Project Public
# License from CTAN archives in directory  macros/latex/base/lppl.txt.
# Either version 1.3 or, at your option, any later version.

.PHONY: listings pdf pdf-devel all

listings: listings.sty

pdf: listings.pdf

pdf-devel: listings-devel.pdf

all: listings pdf pdf-devel


listings.sty: listings.dtx listings.ins lstdrvrs.dtx
	tex listings.ins

listings.pdf: listings.sty
	rm -f ltxdoc.cfg
	pdflatex listings.dtx
	makeindex -s gind.ist listings
	pdflatex listings.dtx
	pdflatex listings.dtx

listings-devel.pdf: listings.sty
	rm -rf ltxdoc.cfg
	echo "\AtBeginDocument{\AlsoImplementation}" > ltxdoc.cfg
	pdflatex -jobname=listings-devel listings.dtx
	makeindex -s gind.ist listings-devel
	pdflatex -jobname=listings-devel listings.dtx
	pdflatex -jobname=listings-devel listings.dtx
	rm -rf ltxdoc.cfg


==> listings/listings/README <==
Listings package
Copyright 1996--2004 Carsten Heinz (the package)
Copyright 1996--2007 individual authors (language drivers)
Copyright 2006--2007 Brooks Moses (continued maintenance)
Released under the LaTeX Project Public License 1.3 or later

The `listings' package is a source code printer for LaTeX.
You can typeset stand alone files as well as listings with
an environment similar to `verbatim' as well as you can
print code snippets using a command similar to \verb'.
Many parameters control the output and if your preferred
programming language isn't already supported, you can make
your own definition.

